Evaluating the principle of relatedness: Estimation, drivers and implications for policy

A growing body of research documents that the size and growth of an industry in a place depends on how much related activity is found there. This fact is commonly referred to as the "principle of relatedness". However, there is no consensus on why we observe the principle of relatedness, how best to determine which industries are related or how this empirical regularity can help inform local industrial policy. We perform a structured search over tens of thousands of specifications to identify robust -- in terms of out-of-sample predictions -- ways to determine how well industries fit the local economies of US cities. To do so, we use data that allow us to derive relatedness from observing which industries co-occur in the portfolios of establishments, firms, cities and countries. Different portfolios yield different relatedness matrices, each of which help predict the size and growth of local industries. However, our specification search not only identifies ways to improve the performance of such predictions, but also reveals new facts about the principle of relatedness and important trade-offs between predictive performance and interpretability of relatedness patterns. We use these insights to deepen our theoretical understanding of what underlies path-dependent development in cities and expand existing policy frameworks that rely on inter-industry relatedness analysis.

==> tabs/compare_dens_bin.tex <==
\begin{tabular}{l*{7}{c}}
\hline\hline
\textbf{productive unit}   &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\

\hline
\multicolumn{7}{c}{\textit{Effect of density on employment levels}}\\
\hline
establishment &  0.511\sym{***}&       0.318\sym{***}&                     &       0.439\sym{***}&                     &                     \\
                       &  (14.06)         &      (8.03)         &                     &     (11.77)         &                     &                     \\
firm         &  0.0580         &                     &       0.199\sym{***}&                     &       0.306\sym{***}&                     \\
                       &  (1.58)         &                     &      (4.68)         &                     &      (9.32)         &                     \\
city       &                 &       0.378\sym{***}&       0.462\sym{***}&                     &                     &       0.463\sym{***}\\
                       &                 &      (8.67)         &     (10.02)         &                     &                     &      (9.79)         \\
country       &                &                     &                     &       0.186\sym{***}&       0.289\sym{***}&       0.237\sym{***}\\
                       &                 &                     &                     &      (3.48)         &      (6.19)         &      (4.19)         \\
\hline
\(N\)                   & 384,705         &      384,705         &      384,705         &      384,705         &      384,705         &      384,705         \\
\(R^2\)                 & 0.7198         &      0.7324         &      0.7269         &      0.7225         &      0.7142         &      0.7291         \\
\hline 
\multicolumn{7}{c}{\textit{Effect of density on employment growth}} \\
\hline 
 establishment &     0.00345\sym{*}  &     0.00275         &                     &     0.00755\sym{***}&                     &                    \\
               &      (1.98)         &      (1.85)         &                     &      (5.48)         &                     &                    \\
firm           &     0.00576\sym{***}&                     &     0.00357\sym{*}  &                     &     0.00803\sym{***}&                    \\
               &      (3.40)         &                     &      (2.39)         &                     &      (6.49)         &                    \\
 city        &                     &     0.00937\sym{***}&     0.00891\sym{***}&                     &                     &      0.0105\sym{***}\\
               &                     &      (6.16)         &      (5.75)         &                     &                     &      (7.91)        \\
 country       &                     &                     &                     &    0.000895         &    0.000832         &     0.00118        \\
               &                     &                     &                     &      (0.59)         &      (0.60)         &      (0.85)        \\
\hline 
\(N\)          &      245,395         &      245,395         &      245,395         &      245,395         &      245,395         &      245,395 \\
\(R^2\)                 & 0.0682         &      0.0719         &      0.0723         &      0.0671         &      0.0678         &      0.0716         \\
\hline\hline
\end{tabular}

==> tabs/compare_dens_con.tex <==
\begin{tabular}{l*{7}{c}}
\hline\hline
  \textbf{productive unit}          &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
\hline
\multicolumn{7}{c}{\textit{Effect of density on employment levels}}\\

\hline  
establishment  &       0.116         &       0.114\sym{**} &                     &       0.452\sym{***}&                     &                       \\
               &      (1.92)         &      (2.60)         &                     &      (6.81)         &                     &                       \\
firm           &       0.630\sym{***}&                     &       0.207\sym{***}&                     &       0.592\sym{***}&                       \\
               &     (11.70)         &                     &      (4.82)         &                     &     (10.33)         &                       \\
city         &                     &       0.799\sym{***}&       0.733\sym{***}&                     &                     &       0.795\sym{***}  \\
               &                     &     (30.69)         &     (25.86)         &                     &                     &     (23.27)           \\
country        &                     &                     &                     &       0.372\sym{***}&       0.267\sym{***}&       0.129\sym{***}  \\
               &                     &                     &                     &     (17.10)         &     (11.69)         &      (9.53)           \\
\hline\(N\)    &      384,705         &      384,705         &      384,705         &      384,705         &      384,705         &      384,705           \\
\(R^2\)                 & 0.7391         &      0.7861         &      0.7882         &      0.7335         &      0.7471         &      0.7868         \\
\hline 
\multicolumn{7}{c}{\textit{Effect of density on employment growth}} \\ \hline 
establishment &     0.00220\sym{*}  &     0.00378\sym{*}  &                     &     0.00448\sym{*}  &                     &                      \\
              &      (2.32)         &      (2.17)         &                     &      (2.49)         &                     &                      \\
firm          &     0.00777\sym{***}&                     &     0.00728\sym{***}&                     &     0.00773\sym{***}&                      \\
              &      (5.66)         &                     &      (4.96)         &                     &      (5.72)         &                      \\
city        &                     &     0.00583\sym{**} &     0.00428\sym{*}  &                     &                     &     0.00573\sym{**}  \\
              &                     &      (3.10)         &      (2.23)         &                     &                     &      (2.97)          \\
country       &                     &                     &                     &     0.00450\sym{***}&     0.00297\sym{**} &     0.00358\sym{**}  \\
              &                     &                     &                     &      (4.25)         &      (2.74)         &      (2.86)          \\
\hline 
\(N\)         &      245,395         &      245,395         &      245,395         &      245,395         &      245,395         &      245,395          \\
\(R^2\)                 & 0.0684         &      0.0662         &      0.0692         &      0.0656         &      0.0687         &      0.0660         \\
\hline\hline
\end{tabular}

==> tabs/multiden_bin_growth.tex <==
\begin{tabular}{l*{11}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}&\multicolumn{1}{c}{(9)}&\multicolumn{1}{c}{(10)}&\multicolumn{1}{c}{(11)}\\
            &\multicolumn{1}{c}{growth8}&\multicolumn{1}{c}{growth8}&\multicolumn{1}{c}{growth8}&\multicolumn{1}{c}{growth8}&\multicolumn{1}{c}{growth8}&\multicolumn{1}{c}{growth8}&\multicolumn{1}{c}{growth8}&\multicolumn{1}{c}{growth8}&\multicolumn{1}{c}{growth8}&\multicolumn{1}{c}{growth8}&\multicolumn{1}{c}{growth8}\\
\hline
lograw      &     -0.0230\sym{***}&     -0.0228\sym{***}&     -0.0247\sym{***}&     -0.0219\sym{***}&     -0.0231\sym{***}&     -0.0249\sym{***}&     -0.0248\sym{***}&     -0.0230\sym{***}&     -0.0228\sym{***}&     -0.0247\sym{***}&     -0.0248\sym{***}\\
            &    (-24.29)         &    (-24.25)         &    (-26.71)         &    (-23.21)         &    (-24.36)         &    (-26.69)         &    (-26.88)         &    (-24.18)         &    (-24.01)         &    (-26.67)         &    (-26.63)         \\
[1em]
regionsum   &      0.0238\sym{***}&      0.0233\sym{***}&      0.0264\sym{***}&      0.0232\sym{***}&      0.0236\sym{***}&      0.0263\sym{***}&      0.0260\sym{***}&      0.0239\sym{***}&      0.0234\sym{***}&      0.0264\sym{***}&      0.0260\sym{***}\\
            &     (24.43)         &     (23.65)         &     (25.88)         &     (23.43)         &     (24.01)         &     (26.06)         &     (25.49)         &     (24.30)         &     (23.37)         &     (25.96)         &     (25.35)         \\
[1em]
indsum      &      0.0234\sym{***}&      0.0229\sym{***}&      0.0254\sym{***}&      0.0219\sym{***}&      0.0232\sym{***}&      0.0254\sym{***}&      0.0252\sym{***}&      0.0233\sym{***}&      0.0229\sym{***}&      0.0253\sym{***}&      0.0253\sym{***}\\
            &     (15.68)         &     (15.62)         &     (16.10)         &     (14.59)         &     (15.62)         &     (16.10)         &     (15.77)         &     (15.58)         &     (15.63)         &     (15.71)         &     (15.68)         \\
[1em]
$d_{irt}$ plant &     0.00811\sym{***}&                     &                     &                     &     0.00345\sym{*}  &     0.00275         &                     &     0.00755\sym{***}&                     &                     &    0.000616         \\
            &      (7.84)         &                     &                     &                     &      (1.98)         &      (1.85)         &                     &      (5.48)         &                     &                     &      (0.33)         \\
[1em]
$d_{irt}$ firm &                     &     0.00853\sym{***}&                     &                     &     0.00576\sym{***}&                     &     0.00357\sym{*}  &                     &     0.00803\sym{***}&                     &     0.00342         \\
            &                     &      (8.44)         &                     &                     &      (3.40)         &                     &      (2.39)         &                     &      (6.49)         &                     &      (1.91)         \\
[1em]
$d_{irt}$ region &                     &                     &      0.0111\sym{***}&                     &                     &     0.00937\sym{***}&     0.00891\sym{***}&                     &                     &      0.0105\sym{***}&     0.00887\sym{***}\\
            &                     &                     &     (10.53)         &                     &                     &      (6.16)         &      (5.75)         &                     &                     &      (7.91)         &      (5.42)         \\
[1em]
$d_{irt}$ country &                     &                     &                     &     0.00561\sym{***}&                     &                     &                     &    0.000895         &    0.000832         &     0.00118         &   -0.000543         \\
            &                     &                     &                     &      (4.93)         &                     &                     &                     &      (0.59)         &      (0.60)         &      (0.85)         &     (-0.37)         \\
[1em]
\_cons      &      -0.467\sym{***}&      -0.456\sym{***}&      -0.514\sym{***}&      -0.446\sym{***}&      -0.463\sym{***}&      -0.512\sym{***}&      -0.506\sym{***}&      -0.466\sym{***}&      -0.457\sym{***}&      -0.511\sym{***}&      -0.507\sym{***}\\
            &    (-21.59)         &    (-21.15)         &    (-21.87)         &    (-20.45)         &    (-21.19)         &    (-21.74)         &    (-20.93)         &    (-21.57)         &    (-21.17)         &    (-21.50)         &    (-20.82)         \\
\hline
\(N\)       &      245395         &      245395         &      245395         &      245395         &      245395         &      245395         &      245395         &      245395         &      245395         &      245395         &      245395         \\
\hline\hline
\multicolumn{12}{l}{\footnotesize \textit{t} statistics in parentheses}\\
\multicolumn{12}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}

==> tabs/multiden_bin_levels.tex <==
\begin{tabular}{l*{11}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}&\multicolumn{1}{c}{(9)}&\multicolumn{1}{c}{(10)}&\multicolumn{1}{c}{(11)}\\
            &\multicolumn{1}{c}{lograw}&\multicolumn{1}{c}{lograw}&\multicolumn{1}{c}{lograw}&\multicolumn{1}{c}{lograw}&\multicolumn{1}{c}{lograw}&\multicolumn{1}{c}{lograw}&\multicolumn{1}{c}{lograw}&\multicolumn{1}{c}{lograw}&\multicolumn{1}{c}{lograw}&\multicolumn{1}{c}{lograw}&\multicolumn{1}{c}{lograw}\\
\hline
regionsum   &       0.953\sym{***}&       0.948\sym{***}&       1.007\sym{***}&       1.003\sym{***}&       0.952\sym{***}&       0.983\sym{***}&       0.989\sym{***}&       0.968\sym{***}&       0.974\sym{***}&       1.014\sym{***}&       0.995\sym{***}\\
            &     (66.42)         &     (60.38)         &     (62.95)         &     (72.70)         &     (65.13)         &     (59.89)         &     (55.69)         &     (69.44)         &     (65.53)         &     (64.60)         &     (61.14)         \\
[1em]
indsum      &       0.900\sym{***}&       0.888\sym{***}&       0.865\sym{***}&       0.858\sym{***}&       0.898\sym{***}&       0.873\sym{***}&       0.863\sym{***}&       0.880\sym{***}&       0.862\sym{***}&       0.846\sym{***}&       0.862\sym{***}\\
            &     (20.71)         &     (20.20)         &     (18.49)         &     (20.18)         &     (20.45)         &     (19.91)         &     (19.06)         &     (19.40)         &     (19.92)         &     (18.30)         &     (18.39)         \\
[1em]
$d_{irt}$ plant &       0.559\sym{***}&                     &                     &                     &       0.511\sym{***}&       0.318\sym{***}&                     &       0.439\sym{***}&                     &                     &       0.301\sym{***}\\
            &     (23.53)         &                     &                     &                     &     (14.06)         &      (8.03)         &                     &     (11.77)         &                     &                     &      (7.11)         \\
[1em]
$d_{irt}$ firm &                     &       0.483\sym{***}&                     &                     &      0.0580         &                     &       0.199\sym{***}&                     &       0.306\sym{***}&                     &     -0.0725\sym{*}  \\
            &                     &     (20.21)         &                     &                     &      (1.58)         &                     &      (4.68)         &                     &      (9.32)         &                     &     (-2.06)         \\
[1em]
$d_{irt}$ region &                     &                     &       0.586\sym{***}&                     &                     &       0.378\sym{***}&       0.462\sym{***}&                     &                     &       0.463\sym{***}&       0.367\sym{***}\\
            &                     &                     &     (19.91)         &                     &                     &      (8.67)         &     (10.02)         &                     &                     &      (9.79)         &      (7.26)         \\
[1em]
$d_{irt}$ country &                     &                     &                     &       0.484\sym{***}&                     &                     &                     &       0.186\sym{***}&       0.289\sym{***}&       0.237\sym{***}&       0.130\sym{*}  \\
            &                     &                     &                     &     (13.83)         &                     &                     &                     &      (3.48)         &      (6.19)         &      (4.19)         &      (2.14)         \\
[1em]
\_cons      &      -18.01\sym{***}&      -17.81\sym{***}&      -18.19\sym{***}&      -18.07\sym{***}&      -17.97\sym{***}&      -18.02\sym{***}&      -17.97\sym{***}&      -17.94\sym{***}&      -17.80\sym{***}&      -18.03\sym{***}&      -18.02\sym{***}\\
            &    (-31.18)         &    (-30.06)         &    (-28.82)         &    (-32.91)         &    (-30.60)         &    (-29.65)         &    (-28.11)         &    (-31.86)         &    (-32.33)         &    (-29.70)         &    (-29.25)         \\
\hline
\(N\)       &      384705         &      384705         &      384705         &      384705         &      384705         &      384705         &      384705         &      384705         &      384705         &      384705         &      384705         \\
\hline\hline
\multicolumn{12}{l}{\footnotesize \textit{t} statistics in parentheses}\\
\multicolumn{12}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}

==> tabs/multiden_con_growth.tex <==
\begin{tabular}{l*{11}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}&\multicolumn{1}{c}{(9)}&\multicolumn{1}{c}{(10)}&\multicolumn{1}{c}{(11)}\\
            &\multicolumn{1}{c}{growth8}&\multicolumn{1}{c}{growth8}&\multicolumn{1}{c}{growth8}&\multicolumn{1}{c}{growth8}&\multicolumn{1}{c}{growth8}&\multicolumn{1}{c}{growth8}&\multicolumn{1}{c}{growth8}&\multicolumn{1}{c}{growth8}&\multicolumn{1}{c}{growth8}&\multicolumn{1}{c}{growth8}&\multicolumn{1}{c}{growth8}\\
\hline
lograw      &     -0.0219\sym{***}&     -0.0230\sym{***}&     -0.0230\sym{***}&     -0.0219\sym{***}&     -0.0232\sym{***}&     -0.0234\sym{***}&     -0.0240\sym{***}&     -0.0226\sym{***}&     -0.0234\sym{***}&     -0.0233\sym{***}&     -0.0242\sym{***}\\
            &    (-22.65)         &    (-23.75)         &    (-25.58)         &    (-23.20)         &    (-24.19)         &    (-25.85)         &    (-25.87)         &    (-23.24)         &    (-23.70)         &    (-25.71)         &    (-26.05)         \\
[1em]
regionsum   &      0.0241\sym{***}&      0.0251\sym{***}&      0.0247\sym{***}&      0.0223\sym{***}&      0.0255\sym{***}&      0.0255\sym{***}&      0.0261\sym{***}&      0.0238\sym{***}&      0.0248\sym{***}&      0.0242\sym{***}&      0.0259\sym{***}\\
            &     (21.70)         &     (25.01)         &     (25.15)         &     (23.20)         &     (25.45)         &     (25.25)         &     (26.96)         &     (22.28)         &     (24.78)         &     (24.69)         &     (26.80)         \\
[1em]
indsum      &      0.0224\sym{***}&      0.0241\sym{***}&      0.0222\sym{***}&      0.0221\sym{***}&      0.0241\sym{***}&      0.0225\sym{***}&      0.0239\sym{***}&      0.0225\sym{***}&      0.0240\sym{***}&      0.0223\sym{***}&      0.0239\sym{***}\\
            &     (14.67)         &     (15.70)         &     (14.80)         &     (14.69)         &     (15.65)         &     (14.90)         &     (15.48)         &     (14.89)         &     (15.52)         &     (14.96)         &     (15.37)         \\
[1em]
$d_{irt}$ plant &     0.00553\sym{**} &                     &                     &                     &     0.00220\sym{*}  &     0.00378\sym{*}  &                     &     0.00448\sym{*}  &                     &                     &     0.00132         \\
            &      (2.71)         &                     &                     &                     &      (2.32)         &      (2.17)         &                     &      (2.49)         &                     &                     &      (1.42)         \\
[1em]
$d_{irt}$ firm &                     &     0.00870\sym{***}&                     &                     &     0.00777\sym{***}&                     &     0.00728\sym{***}&                     &     0.00773\sym{***}&                     &     0.00639\sym{***}\\
            &                     &      (6.72)         &                     &                     &      (5.66)         &                     &      (4.96)         &                     &      (5.72)         &                     &      (4.29)         \\
[1em]
$d_{irt}$ region &                     &                     &     0.00717\sym{***}&                     &                     &     0.00583\sym{**} &     0.00428\sym{*}  &                     &                     &     0.00573\sym{**} &     0.00338         \\
            &                     &                     &      (4.31)         &                     &                     &      (3.10)         &      (2.23)         &                     &                     &      (2.97)         &      (1.59)         \\
[1em]
$d_{irt}$ country &                     &                     &                     &     0.00556\sym{***}&                     &                     &                     &     0.00450\sym{***}&     0.00297\sym{**} &     0.00358\sym{**} &     0.00194         \\
            &                     &                     &                     &      (5.68)         &                     &                     &                     &      (4.25)         &      (2.74)         &      (2.86)         &      (1.57)         \\
[1em]
\_cons      &      -0.462\sym{***}&      -0.489\sym{***}&      -0.461\sym{***}&      -0.439\sym{***}&      -0.493\sym{***}&      -0.473\sym{***}&      -0.494\sym{***}&      -0.458\sym{***}&      -0.483\sym{***}&      -0.456\sym{***}&      -0.492\sym{***}\\
            &    (-20.06)         &    (-21.67)         &    (-21.21)         &    (-19.88)         &    (-21.91)         &    (-21.28)         &    (-22.08)         &    (-19.97)         &    (-20.91)         &    (-20.83)         &    (-21.46)         \\
\hline
\(N\)       &      245395         &      245395         &      245395         &      245395         &      245395         &      245395         &      245395         &      245395         &      245395         &      245395         &      245395         \\
\hline\hline
\multicolumn{12}{l}{\footnotesize \textit{t} statistics in parentheses}\\
\multicolumn{12}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}

==> tabs/multiden_con_levels.tex <==
\begin{tabular}{l*{11}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}&\multicolumn{1}{c}{(9)}&\multicolumn{1}{c}{(10)}&\multicolumn{1}{c}{(11)}\\
            &\multicolumn{1}{c}{lograw}&\multicolumn{1}{c}{lograw}&\multicolumn{1}{c}{lograw}&\multicolumn{1}{c}{lograw}&\multicolumn{1}{c}{lograw}&\multicolumn{1}{c}{lograw}&\multicolumn{1}{c}{lograw}&\multicolumn{1}{c}{lograw}&\multicolumn{1}{c}{lograw}&\multicolumn{1}{c}{lograw}&\multicolumn{1}{c}{lograw}\\
\hline
regionsum   &       1.085\sym{***}&       1.091\sym{***}&       1.010\sym{***}&       0.930\sym{***}&       1.099\sym{***}&       1.030\sym{***}&       1.039\sym{***}&       1.027\sym{***}&       1.047\sym{***}&       0.996\sym{***}&       1.025\sym{***}\\
            &     (75.65)         &     (94.48)         &    (117.90)         &     (67.21)         &     (83.35)         &    (103.37)         &    (117.49)         &     (73.92)         &     (86.83)         &    (118.17)         &     (94.01)         \\
[1em]
indsum      &       1.034\sym{***}&       1.065\sym{***}&       0.875\sym{***}&       0.874\sym{***}&       1.070\sym{***}&       0.900\sym{***}&       0.923\sym{***}&       0.973\sym{***}&       1.014\sym{***}&       0.866\sym{***}&       0.911\sym{***}\\
            &     (30.98)         &     (35.74)         &     (33.59)         &     (20.00)         &     (36.27)         &     (41.00)         &     (39.81)         &     (29.64)         &     (33.47)         &     (33.57)         &     (41.33)         \\
[1em]
$d_{irt}$ plant &       0.578\sym{***}&                     &                     &                     &       0.116         &       0.114\sym{**} &                     &       0.452\sym{***}&                     &                     &     0.00635         \\
            &      (7.76)         &                     &                     &                     &      (1.92)         &      (2.60)         &                     &      (6.81)         &                     &                     &      (0.16)         \\
[1em]
$d_{irt}$ firm &                     &       0.714\sym{***}&                     &                     &       0.630\sym{***}&                     &       0.207\sym{***}&                     &       0.592\sym{***}&                     &       0.178\sym{***}\\
            &                     &     (11.91)         &                     &                     &     (11.70)         &                     &      (4.82)         &                     &     (10.33)         &                     &      (4.83)         \\
[1em]
$d_{irt}$ region &                     &                     &       0.855\sym{***}&                     &                     &       0.799\sym{***}&       0.733\sym{***}&                     &                     &       0.795\sym{***}&       0.701\sym{***}\\
            &                     &                     &     (26.79)         &                     &                     &     (30.69)         &     (25.86)         &                     &                     &     (23.27)         &     (24.81)         \\
[1em]
$d_{irt}$ country &                     &                     &                     &       0.505\sym{***}&                     &                     &                     &       0.372\sym{***}&       0.267\sym{***}&       0.129\sym{***}&       0.100\sym{***}\\
            &                     &                     &                     &     (19.95)         &                     &                     &                     &     (17.10)         &     (11.69)         &      (9.53)         &      (6.03)         \\
[1em]
\_cons      &      -20.99\sym{***}&      -21.43\sym{***}&      -18.35\sym{***}&      -17.46\sym{***}&      -21.58\sym{***}&      -18.84\sym{***}&      -19.21\sym{***}&      -19.66\sym{***}&      -20.36\sym{***}&      -18.08\sym{***}&      -18.91\sym{***}\\
            &    (-53.45)         &    (-63.66)         &    (-55.31)         &    (-29.85)         &    (-63.08)         &    (-71.46)         &    (-67.23)         &    (-49.11)         &    (-56.23)         &    (-55.61)         &    (-69.25)         \\
\hline
\(N\)       &      384705         &      384705         &      384705         &      384705         &      384705         &      384705         &      384705         &      384705         &      384705         &      384705         &      384705         \\
\hline\hline
\multicolumn{12}{l}{\footnotesize \textit{t} statistics in parentheses}\\
\multicolumn{12}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}

==> tabs/ppml_labor_io2.tex <==
\begin{tabular}{l*{4}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            &\multicolumn{1}{c}{establishment}&\multicolumn{1}{c}{firm}&\multicolumn{1}{c}{region}&\multicolumn{1}{c}{country}\\
\hline
labor2      &       1.100\sym{***}&       0.743\sym{***}&      0.0590\sym{***}&       0.128\sym{***}\\
            &     (23.54)         &     (17.06)         &     (12.96)         &     (12.67)         \\
[1em]
io          &      0.0420\sym{***}&      0.0310\sym{***}&     0.00941\sym{***}&     0.00827\sym{***}\\
            &      (3.41)         &      (3.70)         &      (5.77)         &      (4.40)         \\
[1em]
\_cons      &       4.979\sym{***}&       3.393\sym{***}&       4.382\sym{***}&       2.171\sym{***}\\
            &     (97.14)         &    (227.81)         &   (6608.41)         &   (2003.82)         \\
[1em]
0.src       &           0         &           0         &           0         &           0         \\
            &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
0.trg       &           0         &           0         &           0         &           0         \\
            &         (.)         &         (.)         &         (.)         &         (.)         \\
\hline
\(N\)       &       85464         &       85029         &       85903         &       85903         \\
r2\_p        &       0.810         &       0.774         &       0.861         &       0.456         \\
fixed       &                     &                     &                     &                     \\
\hline\hline
\multicolumn{5}{l}{\footnotesize \textit{t} statistics in parentheses}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}

==> tabs/ppml_labor_io2_copy.tex <==
\begin{tabular}{l*{4}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            &\multicolumn{1}{c}{establishment}&\multicolumn{1}{c}{firm}&\multicolumn{1}{c}{region}&\multicolumn{1}{c}{country}\\
\hline
labor2      &       1.100\sym{***}&       0.743\sym{***}&      0.0590\sym{***}&       0.128\sym{***}\\
            &     (23.54)         &     (17.06)         &     (12.96)         &     (12.67)         \\
[1em]
io          &      0.0420\sym{***}&      0.0310\sym{***}&     0.00941\sym{***}&     0.00827\sym{***}\\
            &      (3.41)         &      (3.70)         &      (5.77)         &      (4.40)         \\
[1em]
\_cons      &       4.979\sym{***}&       3.393\sym{***}&       4.382\sym{***}&       2.171\sym{***}\\
            &     (97.14)         &    (227.81)         &   (6608.41)         &   (2003.82)         \\
[1em]
0.src       &           0         &           0         &           0         &           0         \\
            &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
0.trg       &           0         &           0         &           0         &           0         \\
            &         (.)         &         (.)         &         (.)         &         (.)         \\
\hline
\(N\)       &       85464         &       85029         &       85903         &       85903         \\
r2\_p        &       0.810         &       0.774         &       0.861         &       0.456         \\
fixed       &                     &                     &                     &                     \\
\hline\hline
\multicolumn{5}{l}{\footnotesize \textit{t} statistics in parentheses}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}

==> tabs/ppml_labor_io_copy.tex <==
\begin{tabular}{l*{4}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            &\multicolumn{1}{c}{Establishment}&\multicolumn{1}{c}{Firm}&\multicolumn{1}{c}{City}&\multicolumn{1}{c}{Country}\\
\hline
labor       &       7.344\sym{***}&       2.424\sym{***}&       1.036\sym{***}&       1.114\sym{***}\\
            &      (1.07)         &      (0.24)         &      (0.00)         &      (0.01)         \\
[1em]
io          &       1.056\sym{**} &       1.044\sym{***}&       1.012\sym{***}&       1.014\sym{***}\\
            &      (0.02)         &      (0.01)         &      (0.00)         &      (0.00)         \\
[1em]
0.src       &           1         &           1         &           1         &           1         \\
            &         (.)         &         (.)         &         (.)         &         (.)         \\
[1em]
0.trg       &           1         &           1         &           1         &           1         \\
            &         (.)         &         (.)         &         (.)         &         (.)         \\
\hline
\(N\)       &       85464         &       85029         &       85903         &       85903         \\
r2\_p        &       0.784         &       0.749         &       0.860         &       0.453         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Exponentiated coefficients; Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}

==> tabs/variety_vs_mass_growth.tex <==
\begin{tabular}{l*{9}{c}}
\hline\hline
            &\multicolumn{4}{c}{Binary specifications}&\multicolumn{4}{c}{Continuous Specifications}\\
            &\multicolumn{1}{c}{Establishment}&\multicolumn{1}{c}{Firm}&\multicolumn{1}{c}{Region}&\multicolumn{1}{c}{Country}&\multicolumn{1}{c}{Establishment}&\multicolumn{1}{c}{Firm}&\multicolumn{1}{c}{Region}&\multicolumn{1}{c}{Country}\\
            &\multicolumn{1}{c}{growth8}&\multicolumn{1}{c}{growth8}&\multicolumn{1}{c}{growth8}&\multicolumn{1}{c}{growth8}&\multicolumn{1}{c}{growth8}&\multicolumn{1}{c}{growth8}&\multicolumn{1}{c}{growth8}&\multicolumn{1}{c}{growth8}\\
\hline
lograw      &     -0.0230\sym{***}&     -0.0228\sym{***}&     -0.0247\sym{***}&     -0.0218\sym{***}&     -0.0218\sym{***}&     -0.0229\sym{***}&     -0.0232\sym{***}&     -0.0220\sym{***}\\
            &    (-24.44)         &    (-24.22)         &    (-26.92)         &    (-23.37)         &    (-22.48)         &    (-23.74)         &    (-25.91)         &    (-23.42)         \\
[1em]
regionsum   &      0.0232\sym{***}&      0.0235\sym{***}&      0.0262\sym{***}&      0.0226\sym{***}&      0.0239\sym{***}&      0.0247\sym{***}&      0.0250\sym{***}&      0.0242\sym{***}\\
            &     (22.49)         &     (22.49)         &     (24.69)         &     (22.63)         &     (21.63)         &     (24.35)         &     (25.78)         &     (22.27)         \\
[1em]
indsum      &      0.0236\sym{***}&      0.0228\sym{***}&      0.0255\sym{***}&      0.0223\sym{***}&      0.0228\sym{***}&      0.0243\sym{***}&      0.0225\sym{***}&      0.0225\sym{***}\\
            &     (15.68)         &     (15.11)         &     (15.82)         &     (14.89)         &     (13.35)         &     (15.59)         &     (14.96)         &     (14.60)         \\
[1em]
density\_mass&     0.00748\sym{***}&     0.00893\sym{***}    &     0.0104\sym{***}    &   0.00301      &     0.00376        &    0.00672\sym{***}      &      0.0112\sym{***}     &   0.0130\sym{***}  \\
            &      (6.18)         &      (6.87)       &        (6.07)       &          (1.95)     &      (1.82)        &     (3.97)        &        (3.97)         &      (7.65)         \\
[1em]
density2\_variety&     0.00371\sym{*}  &     -0.00109         &      0.000989       &     0.00391      &      0.00238          &     0.00319         &      -0.00442       &       -0.00875\sym{***}  \\
            &      (1.98)         &       (-0.65)       &          (0.45)      &         (1.95)      &     (1.18)          &      (1.54)          &       (-1.25)       &        (-3.35)       \\
[1em]
\_cons      &      -0.463\sym{***}&      -0.456\sym{***}&      -0.512\sym{***}&      -0.445\sym{***}&      -0.466\sym{***}&      -0.488\sym{***}&      -0.468\sym{***}&      -0.465\sym{***}\\
            &    (-21.87)         &    (-21.05)         &    (-22.17)         &    (-20.71)         &    (-18.95)         &    (-21.81)         &    (-21.50)         &    (-18.77)         \\
\hline
\(N\)       &      245395         &      245395         &      245395         &      245395         &      245395         &      245395         &      245395         &      245395         \\
\hline\hline
\multicolumn{9}{l}{\footnotesize \textit{t} statistics in parentheses}\\
\multicolumn{9}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}

==> tabs/variety_vs_mass_levels.tex <==
\begin{tabular}{l*{9}{c}}
\hline\hline
            &\multicolumn{4}{c}{Binary specifications}&\multicolumn{4}{c}{Continuous Specifications}\\
            &\multicolumn{1}{c}{Establishment}&\multicolumn{1}{c}{Firm}&\multicolumn{1}{c}{Region}&\multicolumn{1}{c}{Country}&\multicolumn{1}{c}{Establishment}&\multicolumn{1}{c}{Firm}&\multicolumn{1}{c}{Region}&\multicolumn{1}{c}{Country}\\
            &\multicolumn{1}{c}{lograw}&\multicolumn{1}{c}{lograw}&\multicolumn{1}{c}{lograw}&\multicolumn{1}{c}{lograw}&\multicolumn{1}{c}{lograw}&\multicolumn{1}{c}{lograw}&\multicolumn{1}{c}{lograw}&\multicolumn{1}{c}{lograw}\\
\hline
regionsum   &       0.965\sym{***}&       0.977\sym{***}&       1.024\sym{***}&       1.011\sym{***}&       1.093\sym{***}&       1.104\sym{***}&       1.032\sym{***}&       0.887\sym{***}\\
            &     (68.78)         &     (59.89)         &     (52.91)         &     (66.45)         &     (74.79)         &     (99.86)         &    (105.60)         &     (37.32)         \\
[1em]
indsum      &       0.900\sym{***}&       0.884\sym{***}&       0.849\sym{***}&       0.852\sym{***}&       1.015\sym{***}&       1.042\sym{***}&       0.875\sym{***}&       0.866\sym{***}\\
            &     (21.34)         &     (21.63)         &     (18.83)         &     (20.47)         &     (45.42)         &     (39.14)         &     (30.20)         &     (19.02)         \\
[1em]
density\_mass&       0.574\sym{***}&       0.533\sym{***}&       0.650\sym{***} &       0.518\sym{***}&       0.663\sym{***}&      0.829\sym{***} &      1.154\sym{***} &    0.338\sym{***}    \\
            &     (20.64)         &      (16.05)        &        (13.85)       &      (13.57)        &        (5.19)       &       (13.39)      &        (21.74)   &      (6.78)        \\
[1em]
density\_variety&   -0.0863\sym{*} &     -0.171\sym{***} &       -0.105         &       -0.0518       &       -0.108        &       -0.161\sym{*}     &    -0.334\sym{***}     &    0.194\sym{*}    \\
            &     (-2.26)         &       (-3.42)       &          (-1.66)     &        (-1.22)      &       (-0.69)       &        (-2.31)       &        (-4.25)      &     (2.57)         \\
[1em]
\_cons      &      -18.14\sym{***}&      -18.08\sym{***}&      -18.19\sym{***}&      -18.08\sym{***}&      -20.87\sym{***}&      -21.30\sym{***}&      -18.57\sym{***}&      -16.90\sym{***}\\
            &    (-34.53)         &    (-36.20)         &    (-28.50)         &    (-32.61)         &    (-66.58)         &    (-66.62)         &    (-45.46)         &    (-22.59)         \\
\hline
\(N\)       &      384705         &      384705         &      384705         &      384705         &      384705         &      384705         &      384705         &      384705         \\
\hline\hline
\multicolumn{9}{l}{\footnotesize \textit{t} statistics in parentheses}\\
\multicolumn{9}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
